Adaptive BPE Tokenization for Enhanced Vocabulary Adaptation in Finetuning Pretrained Language Models

In this work, we show a fundamental limitation in vocabulary adaptation approaches that use Byte-Pair Encoding (BPE) tokenization scheme for fine-tuning pretrained language models (PLMs) to expert domains. Current approaches trivially append the target domain-specific vocabulary at the end of the PLM vocabulary. This approach leads to a lower priority score and causes sub-optimal tokenization in BPE that iteratively uses merge rules to tokenize a given text. To mitigate this issue, we propose AdaptBPE where the BPE tokenization initialization phase is modified to first perform the longest string matching on the added (target) vocabulary before tokenizing at the character level. We perform an extensive evaluation of AdaptBPE versus the standard BPE over various classification and summarization tasks; AdaptBPE improves by 3.57% (in terms of accuracy) and 1.87% (in terms of Rouge-L), respectively. AdaptBPE for MEDVOC works particularly well when reference summaries have high OOV concentration or are longer in length. We also conduct a human evaluation, revealing that AdaptBPE generates more relevant and more faithful summaries as compared to MEDVOC. We make our codebase publicly available at https://github.com/gb-kgp/adaptbpe.

==> latex/relatedworks.tex <==
\section{Related Works}\label{sec:sec_RW}
%To the best of our knowledge, this is the first work to explore vocabulary adaptation strategies for the summarization task. 
Table~\ref{tab:related-work-compare} provides a comparative overview of recent works that have explored vocabulary adaption strategies for classification tasks and domain adaptation techniques for summarization.  

\paragraph{Vocabulary Adaptation Strategies for Classification.} To handle the vocabulary mismatch issue, BioBERT~\cite{cite:BioBert}, retrained the model from scratch using a domain-specific corpus and showed performance improvement over the base pre-trained models. While other works like VOLT~\cite{xu-etal-2021-vocabulary} and AVocaDo~\cite{hong-etal-2021-avocado} aim to optimize the model's vocabulary by adding a set of subwords to the existing vocabulary using some utility scoring function. AVocaDo uses a fragment score-based~\cite{rust-etal-2021-good} threshold, whereas T-DNA~\cite{diao-etal-2021-taming} selects n-grams with high Pointwise Mutual Information and iteratively merges them. exBERT~\cite{tai-etal-2020-exbert} adopts an ad-hoc approach to determine the size of $V_{TGT}$ and fix it as $17K$ ($56$\% of pre-trained vocabulary size), and does not perform any vocabulary optimization.
However, all these vocabulary adaptation works have two major drawbacks: (i) they are limited to classification tasks, and (ii) they show results on a single model type and their algorithm is not flexible enough to handle different model types. To the best of our knowledge, this is the first work that explores vocabulary adaptation strategies for summarization over multiple PLMs. We focus on encoder-decoder-based PLMs because it is computationally infeasible to re-train medical LLMs~\cite{chen2023meditron,wu2023pmcllama}.


\begin{table}[t]
    \centering
    \scriptsize
    \scalebox{0.8}{
    \begin{tabular}{p{2.45cm}p{2.2cm}p{2cm}cc}
    \hline
    \textbf{Related Works}  & \textbf{PLMs} & \textbf{Task} & \textbf{VA} & \textbf{IFT} \\ \hline
    \citet{tai-etal-2020-exbert}  & BERT & Classification & \cmark{} & \xmark{}\\ 
    \citet{diao-etal-2021-taming}  & RoBERTa & Classification & \xmark{} & \xmark{} \\ 
    \citet{hong-etal-2021-avocado}  & BERT & Classification & \cmark{} & \xmark{}  \\
    \citet{healthinf22}  & BERT & Classification & \cmark{} & \xmark{}\\ 
    \citet{xu-etal-2023-retrieval} & BERT & Classification & \xmark{} & \xmark{} \\ \hline
    \citet{xu-etal-2021-vocabulary} & Transformer-Big & Machine Translation & \cmark{} & \xmark{} \\
    \citet{liu2023task} & GPT-2, BART & Question Answering & \cmark{} & \xmark{} \\
    \citet{fabbri-etal-2021-improving}  & BART-L & Summarization & \xmark{} & \cmark{}   \\ 
    \citet{xie2022pre} & BERT & Summarization & \xmark{} & \xmark{} \\  \hline
    \drift{} (Ours)  & BART-L, Pegasus-L, BertSumAbs & Summarization & \cmark{} & \cmark{}  \\ \hline
    
    \end{tabular}
    }
    \caption{Comparison of experimental setup with related works. \textit{VA} stands for \textit{Vocabulary Adaptation} and \textit{IFT} stands for \textit{Intermediate fine-Tuning}. `-L' refers to the \textit{Large} model variant.} %
    \label{tab:related-work-compare}
\end{table}
